Set risk measures

We introduce set risk measures (SRMs), real-valued maps defined on the family of non-empty closed bounded sets of essentially bounded random variables. SRMs extend traditional scalar risk measures by assigning a single capital requirement to an entire set of positions. We develop an axiomatic framework for SRMs, adapting classical properties such as monotonicity, translation invariance, convexity, and positive homogeneity to set arithmetic. The main technical contribution is a dual representation of convex SRMs through the \strict{} topology and regular $\tau$-additive unit-mass measures. We also characterize worst-case SRMs and present examples related to systemic risk, Knightian uncertainty, and preference representations.

==> preamble.tex <==
\usepackage[english]{babel}
\usepackage{lmodern}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{makeidx}
\usepackage{graphicx}
\usepackage{natbib}
\usepackage{har2nat}
\setcitestyle{aysep={,}}
\usepackage[left=.3in,right=.3in,top=.7in,bottom=.7in]{geometry}
\usepackage{float}
\usepackage[dvipsnames]{xcolor}
\RequirePackage[protrusion=true,expansion=true]{microtype}
\usepackage{libertinus}

\usepackage[pagebackref]{hyperref}
\hypersetup{
colorlinks = true,
allcolors = {Blue},
}

% Suppress printed URLs in bibliography; make the whole entry clickable instead
\renewcommand{\harvardurl}[1]{\href{#1}{#1}}
\usepackage{setspace}
\onehalfspacing
\usepackage{nicefrac}

\usepackage{array,longtable}

\usepackage{tikz}
\usetikzlibrary{patterns,positioning, arrows.meta, shadows}

\usepackage[titletoc]{appendix}

\usepackage{keytheorems}
\usepackage{cleveref} % Load AFTER keytheorems if possible, though keytheorems handles order well
\newkeytheorem{Thm}[parent=section, style=definition, name = Theorem]
\newkeytheorem{Prp}[sibling=Thm, style=definition, name = Proposition]
\newkeytheorem{Def}[sibling=Thm, style=definition, name = Definition]
\newkeytheorem{Lmm}[sibling=Thm, style=definition, name = Lemma]
\newkeytheorem{Crl}[sibling=Thm, style=definition, name = Corollary]
\newkeytheorem{Asp}[sibling=Thm, style=definition, name = Assumption]
\newkeytheorem{Exm}[sibling=Thm, style=definition, name = Example]
\newkeytheorem{Rmk}[sibling=Thm, style=definition, name = Remark]

\usepackage{enumerate}
\usepackage[inline]{enumitem}

\renewcommand{\labelenumi}{(\roman{enumi})}

\numberwithin{equation}{section}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\epi}{epi}
\DeclareMathOperator*{\hyp}{hyp}

\NewDocumentCommand{\CB}{O{L^\infty}}{%
\operatorname{CB}(#1)%
}

\newcommand{\cl}{\operatorname{cl}}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\clconv}{\operatorname{clconv}}
\newcommand{\card}{\operatorname{card}}
\newcommand{\Fin}{\operatorname{Fin}}
\newcommand{\K}{\operatorname{K}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\singleton}[1]{\left\lbrace #1 \right\rbrace}
\newcommand{\Rbar}{\overline{\mathbb{R}}}
\newcommand{\CBC}{\operatorname{CBC}}
\newcommand{\defin}{\textbf} % Highlight definitions
\newcommand{\ML}{\operatorname{ML}}
\newcommand{\ES}{\operatorname{ES}}
\newcommand{\EL}{\operatorname{EL}}
\newcommand{\VaR}{\operatorname{VaR}}
\newcommand{\Ent}{\operatorname{S}} % Entropy
\newcommand{\Bor}{\operatorname{Bor}} %\Bor(S) := Borel subsets of S
\newcommand{\interior}{\operatorname{int}}
\newcommand{\Pow}{\mathcal{P}} % power set
\newcommand{\ext}{\operatorname{ext}}
\newcommand{\wc}{WC-boundedness}
\newcommand{\Wc}{WC-bounded}
\newcommand{\intersection}{\cap}

\renewcommand{\le}{\leqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\qedsymbol}{\(\blacksquare\)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Standardized notation %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{mathalfa}
\DeclareMathAlphabet{\mathcalboon}{U}{BOONDOX-cal}{m}{n}
\DeclareMathAlphabet{\mathcalboonbf}{U}{BOONDOX-cal}{b}{n}
\newcommand{\di}{\mathrm{dist}_{\infty}}
\newcommand{\sigmafield}[1]{\mathscr{#1}} % sigma-algebras on \Omega
\newcommand{\rvsetset}[1]{{\mathcalboon{#1}}} % collections of sets of random variables
\newcommand*{\E}[2]{\left\langle #1,#2\right\rangle} % expected value / dual pairing
\newcommand{\R}{\mathbb{R}} % real numbers
\newcommand{\Hlim}{\operatorname{Hlim}}
\newcommand{\Wlim}{\operatorname{Wlim}}
\newcommand{\Wblim}{\operatorname{W_{\it b}lim}}
\newcommand{\tauare}{\boldsymbol{\tau}\mathbf{a}}
\newcommand{\ba}{\mathit{ba}}
\newcommand{\bare}{\mathbf{ba}}
\newcommand{\Ptau}{\mathcalboon{P}^{\tauare}} % regular tau-additive probability measures on the dual unit ball
\newcommand{\Pbare}{\mathcalboon{P}^{\bare}}
\newcommand{\strict}{\textsf{strict}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

